Effect of inhomogeneous surface relaxivity, pore geometry and internal field gradient on NMR logging:exact and perturbative theories and numerical investigations

Nuclear magnetic resonance is widely used as a probe of pore geometry and fluid composition in well logging. One of the critical assumptions often made is that the diffusion of fluid molecules is sufficiently fast to warrant the condition for direct mapping between the surface-enhanced relaxation rate and the pore geometry. In pores satisfying such a condition, but having a significant spatial variation of surface relaxivity (rho), one can show that the one-to-one mapping may break down. The degree to which the NMR logging interpretation is affected has not been systematically studied until now. In this work, we theoretically investigate the interplay between the pore geometry, internal field and the inhomogeneous surface relaxivity. We develop a perturbative framework and compare its results with exact solutions obtained for a class of rho textures in a pore with simple geometry. Its effect is quantified for a wide range of diffusivity and/or rho strength. The result allows us to set the bounds for the change in the final slope of the relaxation curve and may serve as a useful guide for logging applications in real rocks with a wide range of pore sizes and fluid diffusivity. We further employ large scale numerical simulations to perform virtual experiments on more complex situations. Internal field and its gradient distributions were obtained and analyzed for up to 1.5^3 cm^3 based on tomograms of carbonate rocks. We find that the texture of rho based on the internal field gradient induces a small, but observable shift, compared to a random noise generated texture for which no shift is observed.

==> sryu_seg_spwla2009_corrected.bbl.tex <==
\begin{thebibliography}{}
\itemsep0pt

\bibitem[Anand,2007]{Anand:2007p741}
Anand, V. and G. Hirasaki,  2007, Paramagnetic relaxation in sandstones:
  distringuishing t1 and t2 dependence on surface relaxation, internal
  gradients and dependence on echo spacing, SPWLA 48th Annual Logging
  Symposium, 446359V.

\bibitem[Arns,2006]{Arns:2006p581}
Arns, C., A. Sheppard, M. Saadatfar, and M. Knackstedt,  2006, Prediction of
  permeability from NMR response: surface relaxivity heterogeneity, SPWLA 47th
  Annual Logging Symposium,  498610GG.

\bibitem[Bergman,1995]{Bergman:1995p866}
Bergman, D. and K.-J. Dunn,  1995, NMR of diffusing atoms in a periodic porous
  medium in the presence of a nonuniform magnetic field, Physical Review E, {\bf
  52}, 6516.

\bibitem[Brown,1961]{Brown:1961p856}
Brown, R. J.~S.,  1961, Distribution of fields from randomly placed dipoles:
  Free-precession signal decay as result of magnetic grains, Physical Review, {\bf 121}, 1379.

\bibitem[Brownstein,1979]{Brownstein:1979p779}
Brownstein, K. and C. Tarr,  1979, Importance of classical diffusion in NMR
  studies of water in biological cells, Physical Review A, {\bf 19}, 2446.

\bibitem[Cho,2009]{Cho:2009p776}
Cho, H., S. Ryu, J. Ackerman, and Y.-Q. Song,  2009, Visualization of
  inhomogeneous local magnetic field gradient due to susceptibility contrast,
  Journal of Magnetic Resonance, {\bf 198}, 88.

\bibitem[Cohen,1982]{Cohen:1982p593}
Cohen, M. and K. Mendelson,  1982, Nuclear magnetic relaxation and the internal
  geometry of sedimentary rocks, Journal of Applied Physics, {\bf 53}, 1127.

\bibitem[de~Gennes,1982]{deGennes:1982p682}
de~Gennes, P.,  1982, Physics of surfaces and interfaces, C. R. Acad. Sc.
  Paris, {\bf 295}, 1061.

\bibitem[Doussal,1992]{LeDoussal:1992p864}
Doussal, P.~L. and P. Sen,  1992, Decay of nuclear magnetization by diffusion
  in a parabolic magnetic field: An exactly solvable model, Physical Review B, {\bf
  46}, 3465.

\bibitem[Gillis,2002]{Gillis:2002p609}
Gillis, P., F. Moiny, and R. Brooks,  2002, On t2-shortening by strongly
  magnetized spheres: a partial refocusing model, Magnetic Resonance in Medicine, {\bf 47},
  257--263.

\bibitem[Grebenkov,2007]{Grebenkov:2007p774}
Grebenkov, D.,  2007, NMR survey of reflected brownian motion, Reviews of Modern Physics,
  {\bf 79}, 1077--61.

\bibitem[Keating,2007]{Keating:2007p846}
Keating, K. and R. Knight,  2007, A laboratory study to determine the effect of
  iron oxides on proton NMR measurements, Geophysics, {\bf 72}, E27.

\bibitem[Kleinberg,1999]{Kleinberg:1999p868}
Kleinberg, R.,  1999, Nuclear magnetic resonance, Methods in the physics of
  porous media, vol 35.

\bibitem[Kleinberg,1996]{Kleinberg:1996p811}
Kleinberg, R.~L.,  1996, NMR well logging, {\it in} Grant, D.~M. and R.~K.
  Harris, eds., Encyclopedia of Nuclear Magnetic Resonance, John Wiley.

\bibitem[Korringa,1962]{Korringa:1962p646}
Korringa, J., D. Seevers, and H. Torrey,  1962, Theory of spin pumping and
  relaxation in systems with a low concentration of electron spin resonance
  centers, Physical Review, {\bf 127}, 1143.

\bibitem[McCall,1991]{McCall:1991p637}
McCall, K., D. Johnson, and R. Guyer,  1991, Magnetization evolution in
  connected pore systems, Physical Review B, {\bf 44}, 7344.

\bibitem[Ryu,2001]{Ryu:2001p705}
Ryu, S.,  2001, Probing pores using elementary quantum mechanics, Magnetic Resonance Imaging, {\bf 19}, 411.

\bibitem[Ryu,2008]{Ryu:2008p531}
Ryu, S.,  2008, Effects of spatially varying surface relaxivity and pore shape
  on NMR logging, SPWLA Proceedings of the 49th Annual Logging Symposium,
  SPWLA,  737008 BB.

\bibitem[Ryu,2009a]{Ryu:2009p500}
Ryu, S.,  2009a, Effects of inhomogeneous partial absorption and the geometry
  of the boundary on the population evolution of molecules diffusing in general
  porous media, submitted for publication.

\bibitem[Ryu,2009b]{Ryu:2009p753}
Ryu, S. and D. Johnson,  2009b, Aspects of diffusive-relaxation dynamics with a
  {\it non-uniform}, partially absorbing boundary in general porous media,
  submitted for publication.

\bibitem[Sen,1999]{Sen:1999p865}
Sen, P., A. Andre, and S. Axelrod,  1999, Spin echoes of nuclear magnetization
  diffusing in a constant magnetic field gradient and in a restricted geometry,
  Journal of Chemical Physics, {\bf 111}, 6548--6555.

\bibitem[Sheppard,2004]{Sheppard:2004p795}
Sheppard, A., R. Sok, and H. Averdunk,  2004, Techniques for image enhancement
  and segmentation of tomographic images of porous material, Physica A, {\bf
  339}, 145.

\bibitem[Valckenborg,2003]{Valckenborg:2003p867}
Valckenborg, R., H. Huinink, and K. Kopinga,  2003, Nuclear magnetic resonance
  dephasing effects in a spherical pore with a magnetic dipolar field,  Journal of Chemical Physics, {\bf 118}, 3243--3251.

\bibitem[Valfouskaya,2006]{Valfouskaya:2006p549}
Valfouskaya, A., P. Adler, J. Thovert, and M. Fleury,  2006, Nuclear magnetic
  resonance diffusion with surface relaxation in porous media, Journal of Colloid and Interface 
  Science, {\bf 295}, 188.

\bibitem[Wilkinson,1991]{Wilkinson:1991p641}
Wilkinson, D., D. Johnson, and L. Schwartz,  1991, Nuclear magnetic relaxation
  in porous media: The role of the mean lifetime $\tau$ ($\rho$ ,d), Physical Review B,
  {\bf 44}, 4960.

\bibitem[Zielinski,2002]{Zielinski:2002p769}
Zielinski, L., Y.-Q. Song, S. Ryu, and P. Sen,  2002, Characterization of
  coupled pore systems from the diffusion eigenspectrum, Journal of Chemical Physics,
  {\bf 117}, 5361--5365.

\end{thebibliography}

